Meta-Control: Automatic Model-based Control Synthesis for Heterogeneous Robot Skills

The requirements for real-world manipulation tasks are diverse and often conflicting; some tasks require precise motion while others require force compliance; some tasks require avoidance of certain regions, while others require convergence to certain states. Satisfying these varied requirements with a fixed state-action representation and control strategy is challenging, impeding the development of a universal robotic foundation model. In this work, we propose Meta-Control, the first LLM-enabled automatic control synthesis approach that creates customized state representations and control strategies tailored to specific tasks. Our core insight is that a meta-control system can be built to automate the thought process that human experts use to design control systems. Specifically, human experts heavily use a model-based, hierarchical (from abstract to concrete) thought model, then compose various dynamic models and controllers together to form a control system. Meta-Control mimics the thought model and harnesses LLM's extensive control knowledge with Socrates' "art of midwifery" to automate the thought process. Meta-Control stands out for its fully model-based nature, allowing rigorous analysis, generalizability, robustness, efficient parameter tuning, and reliable real-time execution.

==> sec_formulation.tex <==
\section{Formulation}\label{sec:formulation}

In this work, we focus on synthesizing robot skills $\ell_i$, which is defined as a unit action (e.g., grab the eraser, erase the marks)  of a robot task given as a free-form language $\LL$ (e.g. clean the whiteboard)~\cite{huang2023voxposer}. Directly synthesizing controllers from the free-form language is very challenging because the task can contain multiple steps or require contextual understanding. The decomposition $\LL \to \{\ell_1, \ell_2,\dots,\ell_n\}$ is given by a task-level planner, such as an LLM based or a search-based planner. The central problem of this work is to synthesize a control system to accomplish the skill described by $\ell_i$. 

% In the following, we only discuss skill level synthesis and omit the index $i$.

We formulate skill synthesis as a control system synthesis problem.
Control system synthesis is a fundamental aspect of control engineering that involves designing and implementing control systems to manage the behavior of dynamic systems. The goal of control system synthesis is to ensure that a system operates as desired, achieving specified performance criteria such as stability, accuracy, and efficiency. The process typically involves two key steps~\cite{???}, system modelling and controller synthesis. The controller synthesis can be further decomposed into objective design, controller design, and parameter inference. Formally,

Given a system $S$ that takes $n_u$-dimensional control input $u \in U$, with available measurements $y$ of dimension $n_y$. We need to model the system with a dynamic model $f: X\times U \mapsto X$, where the dimension of $X$ is unkown. Then we need to design a controller $\pi: Y \mapsto U$.


% Existing works on LLM for robotics skill synthesis can all fit into this framework. Some methods use LLM for controller objective design with learned controller, some methods use LLM to infer parameter for a given controller template.

Directly designing the control system is very difficult because the designing space is infinite.
Existing work usually simplify the process by different ways, such as inference parameters under a given controller templates~\cite{huang2023voxposer}, choose controller from a predefined controller pool~\cite{}, or 
A proper design scheme that is easy to follow by LLM and covers a wide range of skills is needed.

% \begin{table*}[]
%     \centering
%     \begin{tabular}{ccccc}
%          Method & System Modeling & Control objective & Controller template & Parameter inference\\
         
%     \end{tabular}
%     \caption{Caption}
%     \label{tab:my_label}
% \end{table*}
